Extracting a Knowledge Base of Mechanisms from COVID-19 Papers

The COVID-19 pandemic has spawned a diverse body of scientific literature that is challenging to navigate, stimulating interest in automated tools to help find useful knowledge. We pursue the construction of a knowledge base (KB) of mechanisms -- a fundamental concept across the sciences encompassing activities, functions and causal relations, ranging from cellular processes to economic impacts. We extract this information from the natural language of scientific papers by developing a broad, unified schema that strikes a balance between relevance and breadth. We annotate a dataset of mechanisms with our schema and train a model to extract mechanism relations from papers. Our experiments demonstrate the utility of our KB in supporting interdisciplinary scientific search over COVID-19 literature, outperforming the prominent PubMed search in a study with clinical experts.

==> mechanism/02_intro-old.tex <==
\section{Introduction}
\label{sec:intro}
 \begin{quotation}
\noindent ``Some experts are familiar with one field, such as AI or nanotechnology [...] no one is capable of connecting the dots and seeing how breakthroughs in AI might impact nanotechnology, or vice versa.'' {\textit{--Yuval Noah Harari, Homo Deus, 2016}}
 \end{quotation}
 
% (a) Are mechanism classes (Direct vs. Indirect) important for our last experiments of search quality? if yes, mention it... In all experiments, we have ignored the class label and just focused on identifying relations.  -- \tom{yes, added}

The global effort to mitigate the COVID-19 pandemic  is  an  interdisciplinary  endeavor  with  an intensity the world has rarely seen~\cite{nytimes}.
It is challenging to keep up with the interdisciplinary and rapidly expanding body of research on both past and present findings related to COVID-19 \cite{wang2020cord}. As a recent example, expertise in diverse science and engineering areas enabled a group of 200 scientists to understand airborne transmissibility of the SARS-CoV-2 virus \cite{indoor}.
% In \textit{Homo Deus: A Brief History of Tomorrow} \cite{harari2016homo}, the author writes: ``While some experts are familiar with one field, such as AI, nanotechnology or genetics [...] no one is capable of connecting all the dots and seeing [...] how breakthroughs in AI might impact nanotechnology, or vice versa.'' 
To make progress in connecting research areas, this paper aims at building a knowledge base with a simple unified language capturing diverse relationships between scientific concepts. % based on research spanning virology, physics, epidemiology and building engineering, stating that ``expertise in many science and engineering areas enables us to understand the {\it mechanisms} behind generation of respiratory microdroplets '' \cite{indoor}. 
  %... and how airflow patterns carry microdroplets in buildings
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{mechanism/teaser2.pdf}  
%\includegraphics[width=0.95\linewidth]{mechanism/relstuples2.pdf}
\caption{Our knowledge base of \textit{mechanism} relations spans a wide range of activities, functions, and influences extracted from CORD-19, a corpus of papers related to COVID-19.\tnote{hanna's comment} %\hanna{This figure does not show the coarse-grained nature of mechanisms; proposal, be consistent with  the (Viral mechanism search) figure to show the queries like that figure. Then at the beginning, you can draw E1: x/y/z. E2: w/blah/blah. Then, for specific examples just show the arguments and potentially direct/indirect classses.}
}
    \label{fig:teaser}
\end{figure}

%the primary workhorse of automatic KB construction, has been used to extract \textit{fine-grained} relations, some of which correspond to mechanisms (e.g., chemical-protein regulation) but capture only a fraction of the full breadth of mechanisms in the literature. 
Research in natural language processing has provided resources to understand scientific literature and extract {\it fine-grained} relations in specific research areas such as computer science~\cite{x} or bio-medicine~\cite{x}. In contrast, the interdisciplinary nature of COVID-19 papers requires investigating relationships between scientific concepts not only in the medical domain (e.g., viral binding), but also across different areas (e.g., using image analysis for public health), see Figure~\ref{fig:teaser}. \tom{there's an important point here -- biomedicine is a huge fragmented area, and even within just this "domain", ignoring areas like CS/climatology/etc., we have a lot to contribute by capturing biomed mechanisms that are left uncovered otherwise. }\dan{agree, but not sure how to make the point effectively} Despite this topic diversity, such relations are often described with similar textual phrases across different areas. For example similar language can be used to describe ``a protein used for binding'' or ``image analyses used in public health''.\dan{last sentences seems confused? don't we want to say 'DIFFERENT terminology is used to refer to the same thing? This motivates embedding-based approach. If you really mean to say what is written, one needs to include an example --- i can't think of a phrase that means both binding protein and image analysis}\aida{I think we should say something like this: Similar textual structures are often employed to convey information independent of the domain (e.g. ``a protein \textbf{used in} binding'' or ``image analyses \textbf{used in} public health''). Though the meaning of each phrases(e.g. ``protein'' or ``image analysis'') can assist in determining underlying information where those surface structures are not present.(e.g. ``study of image analyses for face mask detection'')}

In this paper, we define a unified schema to cover  {\it scientific mechanisms} as relationships between diverse scientific concepts, and build a knowledge base (KB)  of {scientific mechanisms} described in the literature related to COVID-19. Our broad schema consists of two coarse-grained relations between generic entities: 
\begin{itemize}
    \item \textit{Direct Mechanisms} (mechanistic activities and functions) which include mentions of mechanistic \textit{activities} (e.g., viral binding) or \textit{functions} engendered by  natural or artificial entities (e.g., a protein used for binding or image analysis used in public health); and also 
    \item \textit{Indirect Mechanisms} (influences and associations) which include \textit{influences and associations} such as possible complications associated with a medical procedure. 
\end{itemize}


Our unified view of  mechanisms strike a balance between fine-grained expressivity achieved by Closed-IE~\cite{Freitag1998TowardGL,Hoffmann2010Learning5R} and breadth achieved by Open IE approaches~\cite{etzioni2008open,stanovsky2018supervised,Zhan2020SpanMF}. Closed-IE approaches rely on fine-grained relation types that do not cover the wide range of relations in the scientific domain. Open-IE approaches focus on general-purpose, schema-free extraction of relations, but many of the relations are generic and uninformative for scientific applications \cite{Kruiper2020_SORE}. 

We collect a dataset of mechanisms (denoted \data---or \textbf{C}OVID-19 \textbf{O}pen \textbf{F}unctional \textbf{I}nformation \textbf{E}xtraction), containing annotated sentences from 250 COVID-19 abstracts with our unified schema. We use our dataset to train an information extraction model.
We apply the learned extractor to CORD-19, a 
large corpus of  papers about COVID-19~\cite{wang2020cord}, to generate a large
knowledge base of 1.5M  mechanism relations  (\kb). We additionally provide search algorithms to answer queries over this KB. 

We evaluate the quality of \kb in three expert studies.\dan{sounds like two studies?} We run search queries on our KB, and find that experts evaluate the returning relations as highly relevant with precision of 85-90\% and recall $\geq 40\%$. Importantly, in a study with MDs actively treating COVID-19 patients and conducting research in this area, our system is found substantially 20\% more useful in terms of search quality and utility, compared to the prominent PubMed KB-powered search engine~\cite{x}. Our main contributions include:

%\begin{itemize}[topsep=1mm,noitemsep]
%    \item We construct and distribute a KB of mechanism relations extracted from COVID-19 literature, based on a novel schema we introduce to generalize across many types of mechanistic activities, functions, influences and associations. We construct \data, and annotated dataset of mechanisms the we use to develop our \kb and to facilitate research in retrieving mechanisms from scientific text.
%     \item We showcase the utility of \kb in answering interdisciplinary scientific search queries in COVID-19 literature, including examples such as climatic effects on SARS-CoV-2 and exploring applications of AI in the CORD-19 corpus. In a study with MDs active in the fight against COVID-19, our system is rated higher than PubMed search in terms of utility and quality.
%\end{itemize}

 % dan's version
\begin{itemize}[topsep=1mm,noitemsep]
    \item We introduce a novel schema for {\em mechanisms} that generalizes across many types of mechanistic activities, functions, influences and associations. We then construct and distribute \data, an annotated dataset comprising 2,730  mechanisms using this schema. % from 250 scientific abstracts, to facilitate research in retrieving mechanisms from scientific text.
    
    \item Using \data, we train a state-of-the-art information extraction system and apply it to 160K abstracts in the COVID-19 literature, constructing \kb, a knowledge-base of 1.5M mechanisms.\footnote{GitHub repository redacted for annonymous review} 
    
    \item We analyze the characteristics and quality of \kb, showing the distribution of relations across scientific subfields and comparing the precision of extracted mechanisms to strong baselines using semantic role labeling. 
    
     \item We showcase the utility of \kb in answering interdisciplinary scientific search queries in COVID-19 literature, including examples such as climatic effects on SARS-CoV-2 and exploring applications of AI in the CORD-19 corpus. In a study with MDs active in the fight against COVID-19, our system is rated higher than PubMed search in terms of utility and quality.
\end{itemize}


% We lay the foundations for the framework, which we hope will open new avenues for knowledge representation and discovery across the sciences.

%We fine-tune a biomedical language model \cite{Gururangan2020DontSP} to capture semantic similarity, and use the model to support semantic neural retrieval over the KB. As far as we are aware, we are the first to propose and construct a comprehensive KB of mechanisms extracted from a large body of interdisciplinary scientific research, where researchers can retrieve structured information on mechanisms from \textit{any} domain, whether cellular-level processes or global impacts. 

%These relationships cover a wide range of concepts in scientific papers -- serving as a {\bf unified language} across many fragmented concepts in the literature, and enabling us to construct a broad-coverage knowledge base -- suitable for the diverse nature of COVID-19 research.

% Scientific papers typically cover topics from diverse domains (e.g., image processing to diagnose lung illness). Additionally, they might include complex concepts (e.g., \textit{...nonviral intratumoral in vivo jet‐injection gene transfer of MIDGE‐hTNF‐alpha...}). 

%Building a comprehensive KB of concepts across the sciences is a daunting task. %Information extraction (IE), the primary workhorse of automatic KB construction, has been used to extract \textit{fine-grained} relations, some of which correspond to mechanisms (e.g., chemical-protein regulation) but capture only a fraction of the full breadth of mechanisms in the literature. %It is challenging to formulate comprehensive fine-grained schemas for diverse domains; 



%In this paper, we strike a balance between expressivity and breadth with a unified view of mechanisms. Our broad schema consists of two coarse-grained relations between generic entities: \textit{direct mechanisms} (mechanistic activities and functions) and \textit{indirect mechanisms} (influences and associations). Using a relation extraction model trained with our schema, we extract 2M mechanism relations. We fine-tune a biomedical language model \cite{Gururangan2020DontSP} to capture semantic similarity, and use the model to support semantic neural retrieval over the KB. As far as we are aware, we are the first to propose and construct a comprehensive KB of mechanisms extracted from a large body of interdisciplinary scientific research, where researchers can retrieve structured information on mechanisms from \textit{any} domain, whether cellular-level processes or global impacts. 



% Successful extraction of mechanisms promises to be useful to researchers in multiple ways.  In a primary class of applications, specifications of mechanisms of interest by researchers might be harnessed to enhance the precision and recall of search and retrieval.  For example, there is an opportunity to increase the precision of retrieval by enabling researchers to further specify a characterization of specific mechanisms of interest. Another direction is the use of the extracted mechanisms to help with discovery of novel methods and approaches via analogical inference that considers relevant mechanisms and findings in literature drawn from other disciplines. Still another application is studying the nature and dynamics of the portfolio of the foci of attention of scientists worldwide on a challenge like COVID-19, to identify coverage, including calling out gaps and opportunities over time.

% Very recently, IE models have been used to extract mentions of entities such as proteins, genes, chemicals and their relations \cite{ilievski2020kgtk,ahamed2020information,hope2020scisight}. This type of information can be stored in a Knowledge Base (KB), supporting structured search queries (e.g., all side-effects of a certain drug). While a primary focus of biomedical IE, this format has important limitations. Papers in any domain often contain mixtures of ideas from many areas (e.g., computational techniques to analyze proteomics data, or image processing to diagnose lung illness). To capture the full breadth and depth of research pertaining to COVID-19, and to be able to find novel cross-domain relations \cite{kittur2019scaling,hope2020scisight}, the space of possible entity and relation types would quickly explode. Indeed, even current biomedical ontologies contain millions of possible types and relations \cite{salvadores2013bioportal}, while current IE methods focus on a relatively tiny portion (such as drugs, proteins, genes, diseases and interventions \cite{wallace2016extracting}); expanding to cover areas such as engineering, physics, computer science or even social psychology and economics would require inordinate resources.

% An orthogonal problem is that scientific work describes complex compositions of entities, functions, processes; automatically disentangling them into entities and relations from a closed vocabulary can be extremely hard, even if such a vocabulary were to exist. Consider the following example: \textit{...nonviral intratumoral in vivo jet‐injection gene transfer of MIDGE‐hTNF‐alpha in combination with vindesine...}; while it mentions multiple ``entities'', it is not clear where one ends and the next begins, and their complex composition as a whole, rather than individual elements, is of interest. 





% \hanna{
% (4) minor editing comment: I propose to use {\small \texttt{entities}} to refer to entities in the text -- entities and main text are getting confused.} 
% \tnote{Dan W: cite (null/novel entities, TAKBP) entity linking, nested entities, hierarchical NER, Design Challenges for Entity Linking https://aiweb.cs.washington.edu/ai/pubs/ling-tacl15.pdf}

% We use a biomedical language model that we fine-tune to capture semantic similarity, build a graph of similar mechanisms and induce concepts by finding cliques. To support search over our KB, we use the same language model for retrieving relations  similar to the query. 

==> mechanism/05res_table.tex <==


%begin{table}[t]
% \setlength{\belowcaptionskip}{-15pt} 
% \centering
% \begin{tabular}{lll} 
% \toprule
% model & Avg. Human & Rouge \\
% \toprule
% DYGIE(\data) & 91.1& 55.2 \\
% SRL &41.7& 22.4\\
% \bottomrule
% \end{tabular}
% \caption{Human evaluation stats for our predictions vs. baseline SRL. We note that human evaluation scores are considerably higher than captured by our automated metrics wrt ground truth annotations, yet still correlated with them - indicating their usefulness in this challenging setting.}
% \label{table:human_pred}
%\end{table}

==> mechanism/1_comments.tex <==
%%% Open comments

% ~\dan{as i understand it, the test set is the union of 50 abstract plus 300 sentences. How many sentences is that? How many relations is that?  This test set is important to establishing the value of \kb\ as a resource, and yet we aren't characterizing it clearly} 

% \hanna{I need one better justification here; like our recall is higher, etc. I like to write down a sentence like this: The results confirm that our approach enables extracting a wider range of relations compared to domain-specific relations, and more precise relations compared to SRL-based methods.}


% \dan{this section is incomplete because it doesn't say how large is the human annotated test set --- this is somehow two paragraphs down in RESULTS?}

% \begin{subfigure}{.38\textwidth}
% \begin{small}
% \begin{tabular}{l|rrr}
% \toprule
% Model &\multicolumn{1}{c}{\textbf{RC}} & \multicolumn{1}{c}{\textbf{RD}} & \multicolumn{1}{c}{\textbf{ED}} \\
% \toprule
% % Model & Substr &  Rouge &    Exact &      Substr &  Rouge &    Exact & Substr &  Rouge &    Exact\\
% \midrule
% OpenIE    &   - &  15.5 & 25.6 \\\
% SRL &    -  &  24.5 &  27.7  \\

% \midrule
% DYGIE(SemRep)   &   6.8 &   8.3 &  32.5   \\
% DYGIE(SciERC) &  18.6 &   20.4 &   39.2  \\
% \midrule

% DYGIE(\data)    &  \textbf{42.8} & \textbf{45.6} &  \textbf{50.2} \\

% \end{tabular}
% \end{small}
% \end{subfigure}

